A Joint PHY and MAC Layer Design for Coded Random Access with Massive MIMO

Grant-free access schemes are candidates to support future massive multiple access applications owing to their capability to reduce control signaling and latency. As a promising class of grant-free schemes, coded random access schemes can achieve high reliabilities also with uncoordinated transmissions and therefore in presence packet collisions. In this paper, an analysis tool for coded random access, based on density evolution, is proposed and exploited for system design and optimization. In sharp contrast with the existing literature, where such tools have been developed under simplified channel assumptions, the proposed tool captures not only MAC layer features, but also the physical wireless fading channel and a realistic physical layer signal processing based on multiple antennas and randomly-chosen orthogonal pilots. Theoretical results are validated by comparison with symbol-level Monte Carlo simulations.

==> Figures/graph_DensityTHR_CRDSA.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
%

\definecolor{brightRed}{rgb}{0.79608,0.26275,0.20784}%
\definecolor{brightBlue}{rgb}{0.20392,0.59608,0.85882}%

\begin{tikzpicture}

\begin{axis}[%
name = boundary,
width=4.521in,
height=3.531in,
at={(0.758in,0.516in)},
scale only axis,
xmin=400,
xmax=700,
xtick distance = 100,
ytick = {1e-6, 1e-5, 1e-4, 1e-3, 1e-2, 1e-1},
yticklabels = {$10^{-6}$, $10^{-5}$, $10^{-4}$, $10^{-3}$, $10^{-2}$, $10^{-1}$},
xlabel style={font=\color{white!15!black}, font = \Large},
xlabel={$K_\mathrm{a}$},
ymode=log,
ymin=1e-06,
ymax=1e-01,
yminorticks=true,
xminorticks = true,
minor tick num = 3,
ylabel style={font=\color{white!15!black}, font = \Large},
ylabel={$P_\mathrm{L}$},
tick label style={black, semithick, font=\Large},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
%yminorgrids,
legend style={at={(0.97,0.03)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% CRDSA 2

\addplot [color=graphGreen, line width=1.2pt, mark size=3.2pt, mark=square, mark options={solid, graphGreen}, forget plot]
  table[row sep=crcr]{%
100	7.55891507331352e-06\\
200	1.71187194308864e-05\\
300	2.48999555357843e-05\\
400	4.00177856825223e-05\\
500	0.000100591715976317\\
600	0.00035591397849466\\
700	0.00148120300751875\\
800	0.00442407407407408\\
900	0.0117578772802653\\
1000	0.0251559701492537\\
1100	0.0462035278154681\\
1200	0.0734791666666667\\
1300	0.104999712973594\\
};\label{crdsa2_sim}
% \addlegendentry{$\Lambda (x) = x^2$}

\addplot [color=graphGreen, dashed, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
596.2195 1e-04\\
596.2195 1e-10\\
};\label{crdsa2_thr}

% Test Error Floor r=2
% \addplot [color=graphGreen, dotted, line width=2.0pt, forget plot]
%   table[row sep=crcr]{%
% 400.0000000000000   0.0000323336169 \\
% 425.0000000000000   0.0000343451893 \\
% 450.0000000000000   0.0000363541564 \\
% 475.0000000000000   0.0000383603672 \\
% 500.0000000000000   0.0000403636712 \\
% 525.0000000000000   0.0000423639185 \\
% 550.0000000000000   0.0000443609594 \\
% 575.0000000000000   0.0000463546452 \\
% 600.0000000000000   0.0000483448275 \\
% 625.0000000000000   0.0000503313584 \\
% 650.0000000000000   0.0000523140908 \\
% 675.0000000000000   0.0000542928781 \\
% 700.0000000000000   0.0000562675745 \\
% };
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% CRDSA 3, N = 78


\addplot [color=brightRed, line width=1.2pt, mark size=3.0pt, mark=o, mark options={solid, brightRed}, forget plot]
  table[row sep=crcr]{%
400	1.37499999997015e-06\\
500	5.1200000000029e-05\\
600	0.000584833333333368\\
700	0.00349271428571429\\
800	0.0129305\\
900	0.0329018888888889\\
};\label{crdsa3_sim}
% \addlegendentry{$\Lambda (x) = x^3$}

\addplot [color=brightRed, dashed, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
545.2918 1e-04\\
545.2918 1e-10\\
};\label{crdsa3_thr}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% CRDSA 4
\addplot [color=brightBlue, line width=1.2pt, mark size=3.7pt, mark=triangle, mark options={solid, brightBlue}, forget plot]
  table[row sep=crcr]{%
300	0\\
400	5.90551181101073e-06\\
500	0.000223350253807153\\
600	0.00241025641025638\\
700	0.0132789115646258\\
800	0.0388333333333334\\
900	0.0821481481481482\\
1000	0.150304761904762\\
1100	0.251311688311688\\
};\label{crdsa4_sim}
% \addlegendentry{$\Lambda (x) = x^4$}

\addplot [color=brightBlue, dashed, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
479.5214 1e-04\\
479.5214 1e-10\\
};\label{crdsa4_thr}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% CRDSA 5

\addplot [color=graphOrange, line width=1.2pt, mark size=3.9pt, mark=diamond, mark options={solid, graphOrange}, forget plot]
  table[row sep=crcr]{%
300	0\\
400	2.59373394966289e-05\\
500	0.000992156862745119\\
600	0.00886507936507941\\
700	0.035\\
800	0.0929404761904762\\
900	0.205640211640212\\
1000	0.377328571428571\\
1100	0.577753246753247\\
};\label{crdsa5_sim}
% \addlegendentry{$\Lambda (x) = x^5$}

\addplot [color=graphOrange, dashed, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
427.1163 1e-04\\
427.1163 1e-10\\
};\label{crdsa5_thr}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\end{axis}

\node[draw,fill=white,inner sep=1.5pt,above left=0.5em] at (boundary.south east){
  {\renewcommand{\arraystretch}{1.2}% for the vertical padding
    \begin{tabular}{ccc}
        $\Lambda(x)$ & \textbf{Sim.} & \textbf{Thr.} \\
        $x^2$ & \ref{crdsa2_sim} & \ref{crdsa2_thr} \\
        $x^3$ & \ref{crdsa3_sim} & \ref{crdsa3_thr} \\
        $x^4$ & \ref{crdsa4_sim} & \ref{crdsa4_thr} \\
        $x^5$ & \ref{crdsa5_sim} & \ref{crdsa5_thr} \\
  \end{tabular}
}};

\end{tikzpicture}%

==> Figures/sim_PLR_IRSAvsCRDSA_mean3.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.15686,0.70588,0.38824}%
\definecolor{mycolor2}{rgb}{0.11765,0.51765,0.28627}%
\definecolor{mycolor3}{rgb}{0.79608,0.26275,0.20784}%
\definecolor{mycolor4}{rgb}{0.57255,0.16863,0.12941}%
\definecolor{mycolor5}{rgb}{0.20392,0.59608,0.85882}%
\definecolor{mycolor6}{rgb}{0.12157,0.38039,0.54510}%

\begin{tikzpicture}

\begin{axis}[%
name = boundary,
width=4.521in,
height=3.531in,
at={(0.758in,0.516in)},
scale only axis,
xmin=0,
xmax=4800,
xminorticks=true,
xtick distance = 800,
ytick = {1e-5, 1e-4, 1e-3, 1e-2, 1e-1, 1},
yticklabels = {$10^{-5}$, $10^{-4}$, $10^{-3}$, $10^{-2}$, $10^{-1}$, $1$},
xlabel style={font=\color{white!15!black}, font = \Large},
xlabel={$K_\mathrm{a}$},
ymode=log,
ymin=1e-05,
ymax=1,
yminorticks=true,
xminorticks=true,
minor tick num = 3,
ylabel style={font=\color{white!15!black}, font = \Large},
ylabel={$P_\mathrm{L}$},
tick label style={black, semithick, font=\Large},
axis background/.style={fill=white},
xmajorgrids,
%xminorgrids,
ymajorgrids,
%yminorgrids,
legend style={at={(0.97,0.03)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% IRSA

\addplot [color=mycolor4, line width=1.2pt, mark size=3.9pt, mark=diamond, mark options={solid, mycolor4}, forget plot, mark repeat = 2]
  table[row sep=crcr]{%
400	0.000110256410256415\\
450	0.000326732673267327\\
500	0.000960416666666686\\
550	0.00235606060606064\\
600	0.00491397849462361\\
650	0.00881210592685999\\
700	0.0157447306791569\\
750	0.0247781420765028\\
800	0.0370143442622951\\
850	0.0512073288331726\\
900	0.0685537340619308\\
% 950	0.0875202761000863\\
% 1000	0.108170491803279\\
};\label{irsa_sim}
% \addlegendentry{$\Lambda(x) = 0.55 \, x^2 + 0.26\, x^3 + 0.19\, x^6$}

\addplot[color=mycolor4, line width = 2.0pt, dashed, forget plot]
table[row sep=crcr]{
428.6057 1e-04\\
428.6057 1e-10\\
};\label{irsa_thr}
% \addlegendentry{\ac{IRSA} \;\;\; - Thr}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Np 64 CRDSA

\addplot [color=mycolor3, line width=1.2pt, mark size=3.0pt, mark=o, mark options={solid, mycolor3}, forget plot]
  table[row sep=crcr]{%
% 400	1.37499999997015e-06\\
% 425	4.11764705887663e-06\\
% 450	9.72222222217489e-06\\
% 475	2.50526315789257e-05\\
500	5.1200000000029e-05\\
% 525	0.000102476190476208\\
% 550	0.00019581818181813\\
% 575	0.00032973913043477\\
600	0.000584833333333368\\
% 650	0.0015535384615385\\
700	0.00349271428571429\\
800	0.0129305\\
900	0.0329018888888889\\
};\label{crdsa_sim}
% \addlegendentry{$\Lambda (x) = x^3$}

\addplot[color=mycolor3, line width = 2.0pt, dashed, forget plot]
table[row sep=crcr]{
545.2918 1e-04\\
545.2918 1e-10\\
};\label{crdsa_thr}
% \addlegendentry{\ac{CRDSA} - Thr}


\addplot [color=mycolor5, line width=1.2pt, mark size=3.0pt, mark=square, mark options={solid, mycolor5}, forget plot]
  table[row sep=crcr]{%
% 2000	5.71428571127797e-08\\
% 2800	6.12244898112735e-08\\
% 3400	8.0580177308498e-08\\
% 3900	1.12399016538589e-07\\
3950    0.00017359327\\
4000	0.00867966374269002\\
4050	0.112083245149912\\
4100	0.355170975609756\\
4150	0.477035180722892\\
4200	0.523117589285714\\
% 4250	0.5545505\\
% 4300	0.582280726744186\\
% 4350	0.606009224137931\\
% 4400	0.626930795454545\\
};\label{crdsa_coll}
%\addlegendentry{CRDSA}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% IRSA

\addplot [color=mycolor6, line width=1.2pt, mark size=3.9pt, mark=triangle, mark options={solid, mycolor6}, mark repeat = 2, forget plot]
  table[row sep=crcr]{%
% 2000	8.91145833333828e-05\\
% 2100	9.47315096251344e-05\\
% 2200	0.000107892107892082\\
% 2300	0.000114057971014492\\
% 2400	0.000125196078431422\\
% 2500	0.00014338823529414\\
% 2600	0.000159781576448248\\
% 2700	0.000171870604781965\\
% 2800	0.00018829113924046\\
% 2900	0.00019520037278653\\
% 3000	0.000228648648648688\\
% 3100	0.000252629253203684\\
%3200	0.000277604166666667\\
%3300	0.000308536064874132\\
3400	0.000369635459817719\\
%3500	0.00042563265306117\\
3600	0.000483015873015913\\
%3700	0.000592126909518265\\
3800	0.000744672657252865\\
%3850	0.000834273044029166\\
3900	0.000976235146966875\\
%3950	0.00116326026551405\\
4000	0.00158131250000004\\
4050	0.00216092592592587\\
4100	0.00330158536585368\\
4150	0.00588728915662651\\
4200	0.0116238705738706\\
4250	0.0240232880844645\\
4300	0.0550354800238522\\
4350	0.125125434718538\\
4400	0.238045920745921\\
};\label{irsa_coll}
%\addlegendentry{IRSA}

\addplot [color=mycolor5, line width=2.0pt, dashed]
  table[row sep=crcr]{%
4076 1e-4 \\
4076 1e-8 \\
};\label{crdsa_coll_thr}

\addplot [color=mycolor6, line width = 2.0pt, dashed]
  table[row sep=crcr]{%
4220 1e-4 \\
4220 1e-8 \\
};\label{irsa_coll_thr}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\end{axis}

\node[draw,fill=white,inner sep=1.5pt,below right=0.5em] at (boundary.north west){
  {\renewcommand{\arraystretch}{1.2}% for the vertical padding
    \begin{tabular}{lccc}
        \textbf{Channel} & \textbf{Distribution} $\Lambda(x)$ & \textbf{Sim.} & \textbf{Thr.} \\
        Realistic &$x^3$ & \ref{crdsa_sim} & \ref{crdsa_thr} \\
        Realistic &$0.55 \, x^2 + 0.26\, x^3 + 0.19\, x^6$ & \ref{irsa_sim} & \ref{irsa_thr} \\
        Collision & $x^3$ & \ref{crdsa_coll} & \ref{crdsa_coll_thr} \\
        Collision & $0.55 \, x^2 + 0.26\, x^3 + 0.19\, x^6$ & \ref{irsa_coll} & \ref{irsa_coll_thr} \\
    \end{tabular}
}};

\end{tikzpicture}%
